Role of Quantum Coherence in Chirped Dynamic Nuclear Polarization

Dynamic Nuclear Polarization (DNP) is transforming NMR and MRI by significantly enhancing sensitivity through the transfer of polarization from electron spins to nuclear spins via microwave irradiation. However, the use of monochromatic continuous-wave (CW) irradiation limits the efficiency of DNP for systems with heterogeneous broad EPR lines. Broad-band techniques such as chirp irradiation offer a solution, particularly for Solid Effect (SE) DNP in such cases. Despite its widespread use, the role of quantum coherence generated during chirp irradiation remains unclear, even though it is a key factor in determining the maximum achievable DNP efficiency. In this work, we use density matrix formalism to provide a comprehensive understanding of the quantum coherence generated during electron-nucleus double-quantum (DQ) and zero-quantum (ZQ) SE transitions and their impact on Integrated Solid Effect (ISE) DNP under chirp irradiation. Our analysis employs fictitious product-operator bases to trace the evolution of electron-nucleus coherence leading to integrated or differentiated SE. We also explore the previously unexamined role of decoherence in optimizing chirped DNP. These findings provide new insights into low-temperature DNP and triplet DNP using photoexcited electrons.

==> comments_notes.tex <==
%\section{SI}

%% we cam add the low boltzmann polarization part...
% However, DNP necessitates low-temperature environments and strong magnetic fields for effective polarization transfer. This is due to the low Boltzmann polarization of electronic and nuclear spins under ambient conditions. One major limitation of DNP-based hyperpolarization methods is that they are impractical for biomedical use. As DNP relies on electron spin polarization in a thermal equilibrium state, it is crucial to operate under high magnetic fields (approximately 7 T) and cryogenic temperatures (around 1 K) to attain nuclear spin polarization levels ranging from a few percent to several tens of percent. Accordingly, it is impossible to obtain spectral information of biomolecules and organisms using DNP.

%Ideally, the width of the field or frequency sweep should be greater than the lifetime of the triplet state and exceed the EPR line width. The enhancement factor for CW SE DNP experiments is inversely proportional to the nuclear Larmor frequency, $\omega_{0n}$, following $\omega_{0n}^{-1}$ or $\omega_{0n}^{-2}$. Consequently, in high-field applications, the CW-DNP regimes exhibit a pronounced reduction in signal enhancement. In contrast, pulsed or time-domain DNP techniques are independent of $\omega_{0n}$, making them a suitable option to improve sensitivity while achieving high-field NMR spectra. \cite{quan2022integrated}

% According to Henstra \textit{et al.}, ISE involves the fast sweep of the magnetic field across the entire EPR spectrum while continuously applying steady continuous-wave (CW) MW irradiation at a fixed frequency. When the microwave power is sufficiently high, each electron spin packet experiences an adiabatic fast passage, leading to the inversion of electron spin polarization. Before this inversion, the condition for flip-flop transitions is met, while after the inversion, the flip-flip transitions occur. As a result, akin to the application of $\pi$-pulses on the electron spin packets, both transitions work together to polarize the nuclear spins instead of acting against each other. This cumulative effect of all spin packets is referred to as the ISE. 

% In contrast, the method introduced by Takeda \textit{et, al.} for the effective DNP through broad EPR electron spins is referred to as Integrated Cross Polarization (ICP) because of its close similarity to the cross polarization technique (CP) in NMR.\cite{takeda2001dynamic}. ICP involves Hartmann-Hahn (HH) locking between electron spins in the rotating frame and nuclear spins in the laboratory frame. By carefully selecting the locking field strength, ICP enables effective polarization transfer between these spins. It uses slow, adiabatic field or frequency sweeps to accommodate the broad EPR linewidth, ensuring that all spin packets remain aligned throughout the process. This method is subtly different from ISE as it does not involve sweeping through the DQ and ZQ matching conditions of every electron spin-packet.

%Choosing a suitable strength for the locking field under SE ensures that the matching condition is satisfied between the electron spin in the rotating frame and the $^1H$ spins in the laboratory frame. This allows for exchange in the spin states between electrons and nuclei, enabling polarization transfer. Due to the broad EPR linewidth, the effective field experienced by each spin packet and its effective precession frequency varies over time. ICP employs field or frequency sweeps that are adiabatically slow to pass through the matching condition for all spin packets simultaneously. The adiabaticity is important to ensure that each spin packet is locked along the effective field in the rotating frame. Additionally, the sweeping must be executed within the lifetime of the triplet state, and the sweeping width should cover the EPR linewidth. As a result, ICP allows for the tapping of larger spin packets, which, in turn, enhances the efficiency of DNP.

%Not rephrased(Takeda): in polycrystalline samples by limiting the sweep range of the magnetic field to a partial area of the broad ESR spectrum. The linewidth is no less than 1 kG due to the large ZFS interaction, and the total area intensity is zero as seen in Fig. 1, so that the ESR spectrum cannot thoroughly be excited. Therefore, in the present experiments we limited the sweep range to the peak width.  only a part of the electron spin packets have been used. Following the laser pulse, the magnetic field is swept from +60G to )60G around the ESR peak shown in Fig. 1 in a period of 15 ls, during which a microwave pulse with an intensity of ca. 5 G is applied; the intensity is adjusted to satisfy the Hartmann±Hahn condition between the electron Zeeman splitting in the rotating frame and the proton Zeeman splitting in the laboratory frame. We call this technique integrated cross polarization +ICP) +originally called integrated solid effect [2]). 

%In Figure \ref{fig:ISE_other_factors}a, a slight change in the applied magnetic field (\textbf{$B_0$}) changes $\omega_{0n}$, this leads to either ISE or DSE. Similarly, minute alterations in k (Figure \ref{fig:ISE_other_factors}b), $\omega_1$ (Figure \ref{fig:ISE_other_factors}c), and $e-n$ orientation ($\beta$) (Figure \ref{fig:ISE_other_factors}d) can lead to either ISE or DSE. Clearly, this effect decreases the net polarization transferred from \textbf{S} to \textbf{I} and subsequently reduces the overall DNP enhancement obtained from ISE or ISE like regimes. 

 \begin{comment}
     The preceding theoretical analysis indicates that the ZQ enhancement is expected to accumulate along with the DQ enhancement due to the adiabatic inversion occurring at $\Omega = 0$. We observe that this effect occurs uniformly across the various spin packets within a broad EPR spectrum. Consequently, fluctuations in the electron Larmor frequency do not result in any anomalies. This is demonstrated in Figure \ref{fig:ISE_broad_EPR} (a, b). Here, the DQ transition induces a negative DNP enhancement, while the ZQ transition produces an additional negative DNP enhancement that builds upon the effects of the DQ transition. This phenomenon is a characteristic feature of ISE-DNP profiles.

%Fig. 3
%Results 1: ISE of Broad EPR


Taking into account various experimental parameters other than the electron Larmor frequency, such as sweep rates, amplitudes, nuclear Larmor frequencies, and $e$-$n$ orientations, we find that an ISE profile may or may not be present. In cases where ISE occurs, we have seen that the ZQ enhancement builds up in the same direction as the DQ enhancement. In contrast, in the absence of ISE, the ZQ compensates for the enhancement of DQ, leading to a reduction in the total DNP transfer. As shown in Figure \ref{fig:ISE_other_factors}(a, b, c, d), even a minor alteration in any of the specified system or experimental parameters can result in DSE. Thus, it becomes clear that the integration of the ZQ transition is inconsistent and the resulting net enhancement from the ZQ transition depends on the parameters mentioned above. This challenges the conventional interpretation of ISE.


%Fig 4
%Results 2: ISE and No ISE cases


We continue our investigation by examining the impact of each DNP transition on the occurrence of ISE. To begin with, we repeatedly sweep the MW offset ($\Omega$) in the DQ transition region. This is achieved by resetting the sweep immediately after the DQ transition occurs. We expect the DQ transition to induce a negative enhancement after each reset. However, performing such a sweep interestingly resulted in the accumulation of both positive and negative enhancements over time, as demonstrated in Figure \ref{fig:ISE_cts_sweep} (a, b). This suggests that throughout the DQ transition, the density matrix undergoes complex changes, with both populations and coherences evolving dynamically. As the DQ transition takes place, the adiabatic chirp generates coherences among the various energy levels within the system. The off-diagonal elements of the density matrix, representing these coherences, are pivotal for the integration effect. Additionally, the relative phases of these coherences can cause either constructive or destructive interference, resulting in the observed positive and negative enhancements in the ISE signal when the offset is continuously swept through the DQ transition.

% fig 5:
% continuous sweep across DQ
\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{Figures/Mayur/FIG_7.png}
    \caption{(a) Repeated sweeping through the DQ matching condition to observe the direction of (b) enhancement build-up }
    \label{fig:ISE_cts_sweep}
\end{figure}


In the next section, we describe how the coherences associated with the DQ and ZQ transitions affect the dynamics of a coupled $e-n$ system subjected to a MW chirp within the ISE frequency range.

\subsection{Analytical Results}

In this part, we consider DQ and ZQ DNP transitions as distinct subspaces utilizing the PSB outlined in Sec. 2. Since the DQ transition happens initially in a frequency-swept setting, we start by examining the DQ sub-matrix.

The DQ transition occurs between the $\ket{\alpha\alpha}$ and $\ket{\beta\beta}$ states in the dipolar-coupled $e-n$ system. The populations and coherences that govern this transition are, respectively, $\rho_{(1,1)},  \rho_{(4,4)}$ and $ \rho_{(1,4)}, \rho_{(4,1)}$. In the operator form, the populations are represented by $I_z^{14} = 0.5(S_z + I_z)$ whereas, the real and imaginary parts of the coherences are $I_x^{14} = S_xI_x - S_yI_y$ and $I_y^{14} = S_xI_y + S_yI_x$. As $\omega_{eff}(t)$ approaches $-\omega_{0n}$, the DQ coherences $I_x^{14}$ and $I_y^{14}$ build up leading to the DQ transition. This is observed in Figure \ref{fig:coherence_evolution}(1a, 2a).

\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{Figures/Mayur/FIG_10.png}
    \caption{Evolution of the density matrix during (1) ISE, (2) DSE. For both (1) and (2), (a) DQ coherences, (b) ZQ coherences, (c) DNP profile.}
    \label{fig:coherence_evolution}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale = 0.5]{Figures/Mayur/FIG_11.png}
    \caption{Evolution of the density matrix during (1) ISE, (2) DSE. For both (1) and (2), (a) DQ coherences, (b) ZQ coherences, (c) DNP profile.}
    \label{fig:coherence_evolution}
\end{figure}
% Offset = 0

As discussed previously, at $\Omega = 0$, the maximum inversion of the z-axis magnetization of the electron spin occurs. Accordingly, the DQ coherences transfer to the ZQ coherences. This is clearly observed in Figure \ref{fig:coherence_evolution} (1a, 1b, 2a, 2b), where the oscillations between $I_x^{14}$ and $I_y^{14}$ decay to give rise to oscillations between $I_x^{23}$ and $I_y^{23}$. This is a critical moment in the sweep.
% ZQ transition
Aftermath, the ZQ coherences ($I_x^{23}$ and $I_y^{23}$) continue to build up till a time $t$ such that $\omega_{eff}(t) = \omega_{0n}$ (Figure \ref{fig:coherence_evolution}(1b, 2b)). Figure \ref{fig:zoomed_coherence_evolution}(1a, 2a) shows that, at this point, if $I_y^{23} > I_x^{23}$, ISE occurs (Figure \ref{fig:zoomed_coherence_evolution}(1b)), otherwise, DSE occurs ((Figure \ref{fig:zoomed_coherence_evolution}(1b)). Hence, the attenuation of the transverse coherences formed at the DQ transition is necessary before they can be transferred to their ZQ counterparts when $\Omega = 0$. 

% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.5]{Figures/Mayur/FIG_12.png}
%     \caption{(1)(a)When the coherence $I_y^{23}$ is greater than $I_x^{23}$ at $\omega_{eff}(t) = \omega_{0n}$, (b) ISE occurs. (2)(a) Otherwise, if $I_y^{23}$ is smaller than $I_x^{23}$ at $\omega_{eff}(t) = \omega_{0n}$, (b) DSE occurs.}
%     \label{fig:zoomed_coherence_evolution}
% \end{figure}

Consequently, we consider the effect of $T_2$ relaxation, which dephases the coherences that cause ISE, and are responsible for the caveat between the ISE and the DSE. $T_2$ relaxation is a process that describes the decay of coherences over time due to interactions with the environment or other parts of the system. It is also known as spin-spin relaxation, making it different from spin-lattice relaxation ($T_1$). Incorporating $T_2$ relaxation into the analysis allows us to understand how decoherence is crucial for consistently achieving ISE. For relaxation times $T_2$ ranging from one to a few hundred $\mu s$, ISE is consistently observed at different amplitudes, sweep rates, nuclear Larmor frequencies and $e-n$ orientations, with a single case shown in Figure \ref{fig:ISE_with_T2}(a). In this situation, ISE is absent when $T_2$ is ignored but appears when $T_2$ is shorter than $t$, satisfying condition $\omega_{eff}(t) = \omega_{0n}$. Hence, it can be inferred that for consistent ISE achievement, the relaxation $T_2$ must be optimal, slow enough to allow the DQ coherences to accumulate, yet sufficiently fast to dissipate the coherences prior to the ZQ transition, as illustrated in Figure \ref{fig:ISE_with_T2}(b).



%% Requires completion

% \subsection{Remarks on ASE and SSE}

% Proposed in 2018 \cite{can2018frequency}, and 2020 \cite{tan2020adiabatic}, there are two ISE-like effects that can occur when DNP is performed using an adiabatic MW chirp: ASE and SSE, respectively. In this section we discuss ASE and SSE by building upon the theoretical description of ISE given before.

%% Requires completion
% \newpage
 \end{comment}

%Although DNP techniques using SE result in a significant increase in NMR sensitivity, there are inherent limitations. These limitations encompass paramagnetic broadening \cite{marin2019selective}, stringent barriers to nuclear spin diffusion \cite{stern2021direct}, high costs associated with necessary cryogenics, restricted applicability to biological samples \cite{li2021solid}, biocompatibility concerns \cite{mieville2010scavenging}, and most critically, the limited electron spin polarization at thermal equilibrium.\cite{abhyankar2021challenges} 
%First, the presence of unpaired electron spins in paramagnetic centers leads to faster relaxation of hyperpolarized nuclear spins. This restricts their application in high-resolution spectroscopy.\cite{marin2019selective} Moreover, since DNP depends on the Boltzmann distribution of electron spins at thermal equilibrium, it results in low polarization at ambient conditions.\cite{abhyankar2021challenges} As a result, in DNP, it is crucial to operate under high magnetic fields (approximately 7 T) and cryogenic temperatures (around 1 K) to attain nuclear spin polarization levels ranging from a few percent to several tens of percent. Thus, the high costs associated with the complex cryogenic equipment required for DNP and the impracticality of cryogenic conditions for many biological applications further limit its use. In addition, the reactive and toxic nature of the paramagnetic centers also negatively impacts cell viability and functionality, restricting in-vivo DNP applications.\cite{mieville2010scavenging,tagami2023design}

%Hence, room-temperature DNP methods that utilize biocompatible paramagnetic centers are a highly desirable solution. Hyperpolarization techniques which employ chromophores capable of generating a triplet state upon photoexcitation play a significant role in room-temperature DNP applications.\cite{deimling1980microwave,eills2023spin} One advantage of using the photoexcited triplet state is its transient nature. A transient triplet state has a sufficient lifetime to facilitate electron-to-nucleus DNP transfer. Once the transient is over and the paramagnetic triplet excited state returns to the diamagnetic singlet ground state, the nuclear spins are no longer influenced by the paramagnetic effects. In addition, photoexcited triplet states exhibit a non-degenerate population across different triplet sublevels, independent of temperature and magnetic fields, resulting in a non-equilibrium polarization even at room temperature. This occurs through a spin-selective intersystem crossing (ISC) facilitated by spin-orbit coupling.\cite{henstra1988enhanced,takeda2009triplet} % \cite{schlag1971lifetimes} 
%However, even without the presence of an external magnetic field, the energy-level degeneracy of triplet sublevels is lifted. This is due to an anisotropic interaction known as zero-field splitting (ZFS). ZFS is caused by the dipolar coupling between the two electron spins in the triplet state. 

%The pronounced ZFS anisotropy in a polycrystalline sample leads to inhomogeneously broad electron paramagnetic resonance (EPR) spectral lines. This broadening occurs along with the influence of hyperfine coupling interactions with the surrounding nuclear spins. Consequently, the system exhibits multiplet polarization that encompasses both absorption and emission.\cite{takeda2001dynamic} This is illustrated in Figure \ref{fig:introduction_fig} a. 

%Therefore, room-temperature DNP methods that utilize biocompatible paramagnetic centers are a highly desirable solution. Hyperpolarization techniques that employ chromophores capable of generating a triplet state upon photoexcitation play a significant role in room temperature DNP applications.\cite{deimling1980microwave,eills2023spin}  

%______________________________________________________________________________________


% \subsection{MW Chirp Offset Range I}

% In segment I, if the transfer of polarization from \textbf{S} to \textbf{I} through the DQ transition is adiabatic, then the magnetization vector in the DQ subspace rotates from $DQ_z$ to $-DQ_z$, as shown in Figure \ref{fig:Adiabatic_DSE}a, similar to the single spin-1/2 system \textbf{S} described in Figure \ref{fig:Adiabatic} a(ii, iii), Sec. \ref{sec:Adiabatic Inversion}. 

% However, if the transfer of polarization in this region of the chirp is non adiabatic (w.r.t. the DQ transition), then the density matrix in the DQ subspace comprises of both polarization and coherence after the DQ transition occurs as shown in Figure \ref{fig:ISE_subspaces} (a(i), b(i)). This leads to the magnetization vector pointing in the equatorial region as seen in the Bloch sphere in Figure \ref{fig:bloch_ise_dse}(a, c) analogous to Figure \ref{fig:Adiabatic} (c), Sec. \ref{sec:Adiabatic Inversion}.

% In general, achieving an adiabatic DNP transition is impractical. This is because the effective perturbation that causes the DQ transitions is small, given by a factor $\frac{B\omega_1}{\omega_{0n}}$, as $B \ll \omega_{0n}$ as compared to EPR transitions, as seen in Equation \ref{subspace_Hamiltonian} and \ref{chirp_DNP_Hamiltonian}.

% \subsection{MW Chirp Offset Range II}

% \begin{figure}
%     \centering
%     \includegraphics[scale = 0.55]{Figures/Mayur/FIG_9.png}
%     \caption{When the sweep through both DNP transitions (DQ and ZQ) is adiabatic, (a) no net transverse magnetization evolves in the DQ basis, (b) therefore, no coherences are transferred to the ZQ subspace. Thus, (c) the all polarization adiabatically transfers from $S$ to $I$ during the DQ transition and back from $I$ to $S$ during the ZQ transition. Sweep range: $-200 MHz$ to $200 MHz$, $\omega_{0n} = 100 MHz$, $\omega_1 = 30 MHz$, $k = 0.3 MHz/\mu s$, $B = 2.25 MHz$}
%     \label{fig:Adiabatic_DSE}
% \end{figure}


% If the sweep through the former range is non-adiabatic with respect to the DQ transition, the range is swept with some coherence initially present in the DQ subspace. If the MW chirp pulse is adiabatic w.r.t. the inversion of $S_z$, we observe the complete inversion of the $S_z$ magnetization, and the coherences in the DQ subspace are symmetrically transferred to those of the ZQ subspace.  Thus, at the end of this range, the coherences of the ZQ subspace, i.e., $ZQ_x$ and $ZQ_y$, have a reasonable amplitude (Figure \ref{fig:ISE_subspaces}a(ii), b(ii)); and the magnetization vector in the ZQ basis points in the equatorial region even before the ZQ transition occurs.  

% However, if the MW chirp pulse in this range is non-adiabatic (w.r.t. to inversion of $S_z$), as discussed in Figure \ref{fig:Adiabatic}c(iii), Sec. \ref{sec:Adiabatic Inversion}, it fails to achieve full inversion of the $S_z$ magnetization. This results in the partial transfer of coherences from the DQ subspace to the ZQ subspace. 
 
% \subsection{MW Chirp Offset Range III}
% If the sweep through the first offset range is non-adiabatic (w.r.t. DQ transition), and the second range is adiabatic (w.r.t. inversion of $S_z$); a non-adiabatic sweep (w.r.t. ZQ transition) through this range can lead to either positive or negative z-axis magnetization in the ZQ subspace as represented in Figure \ref{fig:bloch_ise_dse}(b, d). 
% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale = 0.48]{Figures/Mayur/FIG_8.png}
%     \caption{This figure illustrates how the net magnetization vector evolves during ISE in panels (a) for the DQ subspace and (b) for the ZQ subspace, as well as during DSE in panels (c) for the DQ subspace and (d) for the ZQ subspace. Importantly, the magnetization vector in the ZQ subspace can have a net negative z-component leading to ISE, or a net positive z-component leading to DSE. Sweep range: $-200 MHz$ to $200 MHz$, $k = 1 MHz/\mu s$, $\omega_{0n} = 100 MHz$, $B = 2.25 MHz$, $\omega_1 (ISE) = 25.15 MHz$, and $\omega_1 (DSE) = 25 MHz$ }
%     \label{fig:bloch_ise_dse}
% \end{figure}

% This is because the adiabatic inversion of spin \textbf{S} transferred the coherence from the DQ to the ZQ subspace. As a result, the magnetization vector points in the equatorial region of the Bloch sphere even before the ZQ transition as shown in Figure \ref{fig:bloch_ise_dse}(b, d). 

% Since the initial density matrix in the basis of this transition comprises of both polarization and coherence, a non-adiabatic MW chirp pulse through the matching condition would yield two cases (i) polarization transfer from \textbf{S} to \textbf{I} (equivalent to +z magnetization), or (ii) polarization transfer from \textbf{I} to \textbf{S} (equivalent to -z magnetization). This is analogous to the case observed in Figure \ref{fig:adia_non_adia_Sz}(c, d, e, f) in Sec. \ref{sec:Adiabatic Inversion} for a single spin-1/2 system, and is the cause of the caveat. In such a case, we observe that: when $ZQ_y$ is greater than $ZQ_x$, ISE occurs (Figure \ref{fig:ISE_subspaces}(a(ii (zoomed in), iii)); otherwise, DSE occurs (Figure \ref{fig:ISE_subspaces}(b(ii (zoomed in), iii)). Importantly, the coherences before the ZQ transition are responsible for the caveat observed.

% Interestingly, if the sweep is adiabatic through all possible transitions, we always observe DSE (Figure (\ref{fig:Adiabatic_DSE}(c)). This is because all the polarization first adiabatically transfers from \textbf{S} to \textbf{I} (Figure \ref{fig:Adiabatic_DSE}(a)) during the DQ transition, and then back from \textbf{I} to \textbf{S}(Figure \ref{fig:Adiabatic_DSE}(b)). 

% Experimentally, the case where the DQ and the ZQ transitions are non-adiabatic while the inversion of spin \textbf{S} is adiabatic is the only possible case. This is because DNP transitions are quantum mechanically forbidden. As a result, they require a comparatively slower rate or a greater MW power (than SQ transitions) to maintain adiabaticity which cannot be achieved in practice due to the constraints posed by AWGs.



\begin{comment}
For an $e-n$ system, the static Hamiltonian governing the SE in the laboratory frame is given by
\begin{equation}\label{se_H}
    H_0 = \omega_{0e}S_z -\omega_{0n}I_z\\ + AS_zI_z + BS_zI_x 
    %+\omega_1cos(\omega_{$\mu w$} t +\phi) S_x \\
\end{equation}
where $\omega_{0e}$, $\omega_{0n}$ denote the electron and the nuclear Larmor frequencies respectively. 
%$\omega_1$, $\omega_{$\mu w$}$ and $\phi$ are the power (amplitude), frequency, and phase of the applied $\mu w$.
The coefficients $A$ and $B$ represent the secular and pseudo-secular hyperfine coupling (HFC) terms, respectively, between electron and nuclear spins. The term $B$ is anisotropic and can be described by angle $\beta$ with respect to the external magnetic field.  
The $\mu w$ Hamiltonian in the lab frame is given by: 
\begin{equation}
\nonumber H_{\mu w}=\omega_1cos(\omega_{\mu w} t +\phi) S_x
\end{equation}
where $\omega_1$, $\omega_{\mu w}$, and $\phi$ represent the amplitude, frequency, and phase of the applied $\mu w$, respectively. The pseudo-secular hyperfine coupling term $B$, combined with $\mu w$ irradiation, facilitates the excitation of DQ and ZQ DNP transitions via flip-flip or flip-flop interactions, when offset $\Omega = \pm \omega_{0n}$ (Figure \ref{fig:introduction_fig} (c)) as will be delineated below using the appropriate frame transformation. 

In the electron Larmor-frame, the $\mu w$ Hamiltonian is given by $\Tilde{H}_{\mu w}$=$\omega_1 S_x$. By transforming this into the eigenframe of the Hamiltonian, $H_0$, the total $e$-$n$ Hamiltonian can be further represented as described in Corzilius \textit{et al}, and Hu \textit{et al}. \cite{corzilius2012solid, hu2011quantum}:
\begin{equation}\label{subspace_Hamiltonian}
    \Tilde{H} = \Omega S_z - \omega_{0n} I_z + AS_zI_z + \frac{\omega_1 B}{4\omega_{0n}}[(S^+ I^- + S^- I^+) -(S^+ I^+ + S^- I^-)] + \frac{\omega_1}{2} (S^+ + S^-)
\end{equation} Using $S_z = \frac{1}{2}(S_z + I_z) +  \frac{1}{2}(S_z - I_z)$, and $\Omega S_z - \omega_{0n} I_z = \frac{1}{2}[(\Omega - \omega_{0n})(S_z + I_z) + (\Omega + \omega_{0n})(S_z - I_z)]$, $\Tilde{H}$ can be rewritten as:
\begin{align}
\Tilde{H}= & \frac{1}{2} \left[\left(\Omega-\omega_{0n}\right)\left(S_{z}+I_{z}\right) + A\left(S_{z}+I_{z}\right)I_{z} - \frac{\omega_{1} B}{2 \omega_{0n}}\left(S^{+}I^{+} + S^{-}I^{-}\right)\right] \nonumber \\
& + \frac{1}{2} \left[\left(\Omega+\omega_{0n}\right)\left(S_{z}-I_{z}\right) + A\left(S_{z}-I_{z}\right)I_{z} + \frac{\omega_{1} B}{2 \omega_{0n}}\left(S^{+}I^{-} + S^{-}I^{+}\right)\right] \nonumber \\
& + \frac{\omega_{1}}{2}\left(S^{+} + S^{-}\right)
\tag{3}
\end{align}
%The effect of the single quantum (SQ) coherences contributing EPR transitions are not considered in this discussion, based on the assumption that their transverse relaxation is faster compared to the DNP transfer. 
We can decompose $\Tilde{H}$ into two commuting subspaces in terms of DQ and ZQ bases using the spin operators corresponding to the DQ transitions ($DQ_X = S_xI_x - S_yI_y$, $DQ_Y = S_xI_y + S_yI_x$, $DQ_Z = \frac{1}{2}(S_z + I_z)$) and the ZQ transitions ($ZQ_X = S_xI_x + S_yI_y$, $ZQ_Y = S_xI_y - S_yI_x$, $ZQ_Z = \frac{1}{2}(S_z - I_z)$), whereas the last term indicates the excitation of the EPR (SQ) transition.
\end{comment}

% The effective SE Hamiltonian is then utilized to understand the transition probabilities of the DNP transitions during the Chirp, along with their impact on the evolution of the density matrix, including polarization and coherence. Subsequently, we unfold the role of coherence in determining the Chirp DNP efficiency.
